Soft Hybrid Aerial Vehicle via Bistable Mechanism

Unmanned aerial vehicles have been demonstrated successfully in a variety of tasks, including surveying and sampling tasks over large areas. These vehicles can take many forms. Quadrotors' agility and ability to hover makes them well suited for navigating potentially tight spaces, while fixed wing aircraft are capable of efficient flight over long distances. Hybrid aerial vehicles (HAVs) attempt to achieve both of these benefits by exhibiting multiple modes; however, morphing HAVs typically require extra actuators which add mass, reducing both agility and efficiency. We propose a morphing HAV with folding wings that exhibits both a quadrotor and a fixed wing mode without requiring any extra actuation. This is achieved by leveraging the motion of a bistable mechanism at the center of the aircraft to drive folding of the wing using only the existing motors and the inertia of the system. We optimize both the bistable mechanism and the folding wing using a topology optimization approach. The resulting mechanisms were fabricated on a 3D printer and attached to an existing quadrotor frame. Our prototype successfully transitions between both modes and our experiments demonstrate that the behavior of the fabricated prototype is consistent with that of the simulation.

==> 2_related_work.tex <==
\section{RELATED WORK}
\subsection{Hybrid Aerial Vehicles (HAVs)}



\subsection{Bistable Mechanism}
Using topology optimization to design bistable structures has been studies for years. The previous work all relied on nonlinear finite element analysis to achieve large deformations, where robustly solving the displacement control and computing the analytic sensitivity information are still challenging. \cite{Prasad2005} maximized the distance between two equilibrium states. But they used a generic algorithm to optimize the topology without sensitivity information, which is not efficient. \cite{James2016} achieved bistability by manipulating the force-displacement curve directly. They minimized the backward switching force and set a lower-bound for the forward switching force. Arc-length method was utilized to achieve displacement control. \cite{Chen2018} followed this formulation, but achieved displacement control by increasing a prescribed displacement gradually to a target displacement. \cite{Chen2019} proposed a new formulation by optimized the range of the force-displacement curve so that two-direction switching forces can be both optimized. We follows this idea as part of our formulation. 
%Besides, in this paper, following LETO \cite{li2020leto}, the governing equation is discretized by Material Point Method (MPM), which directly minimize the strain energy to get equilibrium states. From this point of view, displacement control can be modeled as an energy minimization with an equality constraint, which can be solved using augmented Lagrangian method. With projected Newton method \cite{teran2005robust} that are already utilized in \cite{li2020leto}, the displacement control is very robust and can achieve very large prescribed displacement.

\subsection{Multi-body Mechanism}
We utilize a multi-body mechanism for our wing design to exert large rotations. Our idea stems from \cite{Swartz2019}, which connects layers of FEM meshes with clusters of springs with decayed stiffness to simulate pin joints between layers. The major advantage of this pin joint model is the enforcement of positional continuity, which enables effective numerical optimization. Inspired by this work, we model joints as equality constraints between the interpolated displacements on the same material coordinate of two different layers in our optimization-based equilibrium solver. Consequently, each joint is placed inside a computational cell with it's position optimized.

==> 6_acknowledgement.tex <==
\section*{ACKNOWLEDGMENT}
We would like to thank Jason Friedman for CAD assistance, Yifan Yuan for 3D printing the TPU arms, and Terry Kientz and Jeremy Wang for their assistance with fabricating the HAV and rotating boom. 
